On the Practicality of Atomic MWMR Register Implementations

Multiple-writer/multiple-reader (MWMR) atomic register implementations provide precise consistency guarantees, in the asynchronous, crash-prone, message passing environment. Fast MWMR atomic register implementations were first introduced in Englert et al. 2009. Fastness is measured in terms of the number of single round read and write operations that does not sacrifice correctness. In Georgiou et al. 2011 was shown, however, that decreasing the communication cost is not enough in these implementations. In particular, considering that the performance is measured in terms of the latency of read and write operations due to both (a) communication delays and (b)local computation, they introduced two new algorithms that traded communication for reducing computation. As computation is still part of the algorithms, someone may wonder: What is the trade-off between communication and local computation in real-time systems? In this work we conduct an experimental performance evaluation of four MWMR atomic register implementations: SFW from Englert et al. 2009, APRX-SFW and CWFR from Georgiou at al. 2011, and the generalization of the traditional algorithm of Attiya et al. 1996 in the MWMR environment, which we call SIMPLE. We implement and evaluate the algorithms on NS2, a single-processor simulator, and on PlanetLab, a planetary-scale real-time network platform. Our comparison provides an empirical answer to the above question and demonstrates the practicality of atomic MWMR register implementations.

==> ns2-testbed.tex <==
\paragraph{Experimentation Platform:}
Our test environment consists
of a set of writers, readers, and servers. 
We use bidirectional links 
between the communicating nodes, with 1Mb bandwidth, 
latency of $10ms$, and a DropTail queue.
To model asynchrony, the processes send messages 
after a random delay between 0 and 0.3 $sec$. 
%
%According to our setting,
%only the messages from the invoking processes to the servers,
%and the replies from the servers to the processes are
%delivered (no messages are exchanged among the 
%servers or the invoking processes).
We ran NS2 in Ubuntu,
on a Centrino 1.8GHz processor. The average of 5 samples
per scenario provided the stated operation latencies.
 
We have evaluated the algorithms with majority quorums. 
 As discussed in \cite{EGMNS09}, assuming $|\srvSet|$ servers
 out of which $f$ can crash, we can construct an
 $(\frac{|\srvSet|}{f}-1)$-wise quorum system $\qs$. 
 Each quorum $Q$ of $\qs$ has size $|Q|=|\srvSet|-f$. 
 The processes are not aware of $f$.  The quorum system is 
generated \emph{a priori} and is distributed to each participant 
node via an external service (out of the 
scope of this work). 
%
We model server failures by selecting some quorum of servers 
(unknown to the participants) to be correct and allowing any other server to crash. 
%Note that the non-faulty quorum
%is not known to any of the participants.
The positive time parameter $cInt$ is used to model
the failure frequency or reliability of every server $\srvr$.

We use the positive time parameters $rInt=5sec$ and $wInt=10sec$
 to model operation frequency. Readers and writers pick a uniformly at random 
 time between $[0\ldots rInt]$ and $[0\ldots wInt]$, respectively,
 to invoke their next read (resp. write) operation. 
% the time
%intervals between any two successive read operations
%and any two successive write operations respectively.
%



